LDL: Line Distance Functions for Panoramic Localization

We introduce LDL, a fast and robust algorithm that localizes a panorama to a 3D map using line segments. LDL focuses on the sparse structural information of lines in the scene, which is robust to illumination changes and can potentially enable efficient computation. While previous line-based localization approaches tend to sacrifice accuracy or computation time, our method effectively observes the holistic distribution of lines within panoramic images and 3D maps. Specifically, LDL matches the distribution of lines with 2D and 3D line distance functions, which are further decomposed along principal directions of lines to increase the expressiveness. The distance functions provide coarse pose estimates by comparing the distributional information, where the poses are further optimized using conventional local feature matching. As our pipeline solely leverages line geometry and local features, it does not require costly additional training of line-specific features or correspondence matching. Nevertheless, our method demonstrates robust performance on challenging scenarios including object layout changes, illumination shifts, and large-scale scenes, while exhibiting fast pose search terminating within a matter of milliseconds. We thus expect our method to serve as a practical solution for line-based localization, and complement the well-established point-based paradigm. The code for LDL is available through the following link: https://github.com/82magnolia/panoramic-localization.

==> 1_intro.tex <==
\section{Introduction}

% Visual localization, and potential of panorama images
Estimating the location of a device or agent with respect to a pre-captured 3D map has widespread applications in robotics, AR/VR, and embodied navigation.
Visual localization is a loss-effective localization method that aims to find the location only using image input.
While perspective images are widely used for visual localization, it suffers from challenges in textureless regions, illumination changes and scene object changes.
Panorama images have the potential to overcome such challenges, due to the large field of view that disambiguates such adversaries and provides ample evidence for robust localization.
Recent advances in visual localization using panorama images~\cite{gosma, gopac, piccolo, sphere_cnn} have demonstrated that reasonably robust localization is possible even amidst local scene changes or repetitive structure.
However, as these methods are based on the raw color or light intensity as input, localization performance may deteriorate with drastic changes in illumination or sensor settings such as white balance setting.


% potential of using lines along with challenges
Line segments have a number of desirable properties compared to raw color, semantic labels or learned features commonly used for visual localization~\cite{sarlin2019coarse,gosma,piccolo}.
First, due to the long standing work in line segment extraction~\cite{LSD, lineseg_1, lineseg_2, lineseg_3}, it is cheap and stable to obtain line segments, even amidst dramatic changes in illumination or moderate motion blur.
Second, lines are sparse representations of a scene, and leads to small memory and computation requirement.
Nevertheless, line segments alone are visually ambiguous compared to other localization cues (color, semantic labels, etc.), which is a major bottleneck for successful localization using lines.

% overview of pipeline
In this paper, we propose LDL, a quick and robust algorithm for finding the camera pose from line segments in 2D and 3D.
Given a 2D panorama query image and 3D point cloud as a reference map, we first extract line segments in both modalities using off-the-shelf line detection algorithms~\cite{LSD, 3d_lineseg}.
LDL finds pose through a three-step process that sequentially decodes the spatial context of line segments, as shown in Figure~\ref{fig:overview}.
The localization starts by extracting principal directions of lines in 2D and 3D, from which we reduce the search space of candidate rotations.
Then distance functions are generated from spherical projections of the detected lines for both 2D and 3D, from which we can further deduce a set of translations and rotations.
We enhance the discriminative power of distance functions by decomposition, and separately evaluate lines aligned with each principal directions.
The distance function formulation imbues spatial context even in void regions lacking lines without further processing, in contrast to previous line-based localization approaches~\cite{line_chamfer,line_transformer} that aim to establish correspondences between detected lines.
Since the candidate poses are searched solely using line segments, LDL can rapidly evaluate an immense set of poses within a matter of milliseconds and stay robust to extreme light changes.
As the final step, the selected poses are refined using PnP-RANSAC~\cite{ransac, epnp}, establishing 2D-3D correspondences from a learned feature matching module~\cite{sarlin2020superglue}.

% distance function overview
The key component of LDL is the novel loss formulation using line distance functions, which effectively ranks the candidate poses.
Specifically, we define two separate line distance functions in 2D and 3D, where the function values are evaluated over a spherical surface as shown in Figure~\ref{fig:ldf}.
For an arbitrary point on a sphere, the 2D line distance function is defined as the spherical distance to the closest panorama line segment.
Similarly, the 3D line distance function is defined for each candidate pose as the closest spherical distance to the projected 3D line segments.
Intuitively, one can expect the 2D, 3D distance functions to be similar near the ground-truth pose, as shown in Figure~\ref{fig:ldf}.
Based on this observation, LDL evaluates candidate poses with the affinity of distance functions between 2D and 3D, using a loss function that is robust against object layout changes.
To make the pose selection further discriminative, we decompose the distance functions by clustering lines with principal axes, as shown in Figure~\ref{fig:decomp}.
This offers a sense of ‘direction’ to the distance functions, further disambiguating the line segments and leading to highly accurate candidate pose retrieval.
The distance functions along with its decomposition play a crucial role in robust localization using line segments, which is extensively verified through our experiments.

% performance and overall contribution
LDL is evaluated in various indoor scenes where a few qualitative results are presented in Figure~\ref{fig:qualitative}.
LDL outperforms all tested baselines including existing localization algorithms using line segments, and demonstrates robust performance in scenes with object or illumination changes.
Notably, LDL is extremely light-weight; it does not require pre-computing and caching learned features, or a large set of images with dense groun-truth poses.
Using only sparse line segments, LDL can quickly find a small set initial poses for refinement.
We expect LDL to serve as a practical localization algorithm that could enhance and complement existing visual localization techniques.


==> figures/fig_bar_plot.tex <==
\begin{figure}[t]
  \centering
    \includegraphics[width=\linewidth]{figures/bar_plot.pdf}
   \caption{Privacy-utility curve drawn from various values of $\lambda_\text{2D}{,}\lambda_\text{3D}$ and bar plot showing feature inversion results for object and background regions in the Stanford 2D-3D-S~\cite{stanford2d3d} dataset. }
   \label{fig:barplot}
\vspace{-1em}
\end{figure}

==> figures/fig_deletion.tex <==
\begin{figure}[t]
  \centering
    \includegraphics[width=\linewidth]{figures/deletion.pdf}
    \caption{Deletion of objects and humans in feature inversion attacks after line-based filtering. We further display the inverted PSNR values between the original and filtered inversion results.}
   \label{fig:qualitative}
\vspace{-1em}
\end{figure}

==> figures/fig_overview.tex <==
\begin{figure*}[t]
  \centering
    \includegraphics[width=\linewidth]{figures/overview.pdf}
   \caption{Overview of our approach. LDL first extracts line segments and principal directions from the panorama and point cloud. In addition, our method computes local features~\cite{superpoint} from the panorama and synthetic views in the point cloud, where only features near lines are kept for localization. LDL then selects candidate poses by matching 2D, 3D line distance functions that effectively represent the sparse geometry of lines. Finally, the selected poses are refined via local feature matching~\cite{sarlin2020superglue} near lines and applying PnP-RANSAC~\cite{ransac, epnp}. }
   \label{fig:overview}
\vspace{-1em}
\end{figure*}


==> figures/fig_qualitative.tex <==
\begin{figure}[t]
  \centering
    \includegraphics[width=\linewidth]{figures/qualitative.pdf}
   \caption{Qualitative results of LDL. We show the query image (left), extracted line segment (middle) and the projected point cloud on the estimated pose (right). LDL robustly localizes images containing motion blur, featureless regions, illumination changes or object changes.}
   \label{fig:qualitative}
\end{figure}


==> figures/fig_rotation.tex <==
\begin{figure}[t]
  \centering
    \includegraphics[width=0.9\linewidth]{figures/rotation.pdf}
   \caption{Illustration of estimating the candidate rotations with principal directions. For line segments in 2D and 3D, LDL extracts principal directions using voting. Rotations are estimated for all possible associations between triplets of principal directions.}
   \label{fig:rotation}
\end{figure}

==> figures/fig_server.tex <==
\begin{figure}[t]
  \centering
    \includegraphics[width=\linewidth]{figures/server.pdf}
   \caption{Client-server localization setup using LDL. The mapper and query clients capture the raw 2D, 3D data and share the lines and local features near lines with the service provider. The service provider cannot recover the sensitive visual details as only a fraction of information is shared.}
   \label{fig:server}
\vspace{-1em}
\end{figure}

==> old_files/3_method.tex <==
\section{Method}
\input{figures/fig_motivation}

Given a point cloud $P=\{X, C\}$ with point cloud coordinates $X \in \mathbb{R}^{N\times 3}$ and color values $C \in \mathbb{R}^{N\times 3}$, LDL finds the optimal rotation $R^* \in SO(3)$ and translation $t^* \in \mathbb{R}^{3}$ at which the query image $I$ is taken.
Figure X describes the steps LDL take for localization.
Prior to main localization, LDL extracts lines and principal directions in 2D and 3D, along with local feature descriptors near the line segments (Section~\ref{sec:input prep}).
Then using the principal directions, LDL deduces a set of rotations considering the sign and permutation ambiguity (Section~\ref{sec:rotation}).
Given the set of candidate rotations, we construct an initial set of possible poses incorporating translations. 
We compute line distance functions at each pose and choose the promising poses by comparing the distance functions with a robust loss function (Section~\ref{sec:distance}).
As the final step, we refine the selected poses by performing PnP-RANSAC~\cite{ransac}, where feature matches~\cite{sarlin2020superglue} are found between the cached keypoints lying near 2D and 3D lines (Section~\ref{sec:refinement}).
Due to the line-centric paradigm, the entire localization process of LDL is privacy-preserving (Section~\ref{sec:privacy}).

\if 0
For 2D panoramas we apply LSD~\cite{LSD} to acquire line segments, which is a robust line detection algorithm that can stably extract lines even under motion blur as shown in Figure~\ref{fig:qualitative}.
For 3D point clouds we use the line extraction method from Xiaohu et al.~\cite{3d_lineseg}, which can quickly extract line segments for point clouds containing millions of points within a few seconds.
Given the point cloud with the bounding box size of $b_x \times b_y \times b_z$, we first filter out 3D line segments shorter than the averaged size $(b_x+b_y+b_z)/3$.
The 2D line segments are then filtered with an adaptive length threshold to match the filtering rate of 3D line segments.
Specifically, we choose the threshold value such that the ratio of lines filtered in 2D equals that in 3D.
\fi

\subsection{Localization Input Preparation}
\label{sec:input prep}

\paragraph{Line Segment and Principal Direction Extraction} 
We use off-the-shelf line detection algorithms to obtain line segments in 2D~\cite{LSD} and 3D~\cite{3d_lineseg} from the raw panorama and point cloud.
We use a simple filtering step to remove short, noisy line segments from the raw detection where the details are deferred to the supplementary material.
Using the line detections, LDL extracts the \textit{principal directions} in 2D and 3D by estimating vanishing points and voting for common line directions. 
We use the principal directions to additionally filter line segments whose directions are parallel to the principal directions, and estimate candidate rotations in Section~\ref{sec:rotation}.

In 2D we extract vanishing points by finding the points of intersection of extended 2D line segments.
The 2D principal directions $P_{2D}=\{p\}$ are defined as the top $k_{2D}$ vanishing points containing the most incident lines, where $p \in \mathbb{R}^3$ is a unit norm vector denoting the vanishing point location in the sphere.
Similarly the 3D principal directions $P_{3D}=\{\tilde{p}\}$ are defined as the top $k_{3D}$ most common line directions from 3D line segments obtained via voting.

\paragraph{Line-Based Filtering of Local Feature Descriptors}
For use in pose refinement, LDL caches local feature descriptors of points near the lines in 2D and 3D as shown in Figure X.
In 2D panoramas we first extract local feature descriptors using SuperPoint~\cite{superpoint} and keep descriptors whose distance to the nearest line segment is below a threshold $\lambda_{2D}$.
Specifically, we treat each descriptor location as a point on a sphere and compute the shortest spherical distance between the descriptor and line segments in 2D.

For 3D point clouds we first render synthetic views at $S$ locations using the point cloud color values.
To elaborate, we project the input point cloud $P=\{X,C\}$ on the designated location and assign the measured color $Y(u,v)=C_n$  at the projected location of the corresponding 3D coordinate $(u,v)=\Pi(R X_n + t)$ to create the synthetic view $Y$.
Similar to the 2D case, we then extract local features for each synthetic view $Y$ using SuperPoint~\cite{superpoint}.
Finally, we back-project the local features to their 3D locations and keep local features whose distance to the nearest 3D line segment is below a threshold $\lambda_{3D}$.

\subsection{Candidate Pose Selection}
\if 0
Given a set of 2D and 3D line segments, LDL first estimates a set of feasible rotations by extracting principal directions, as shown in Figure~\ref{fig:rotation}.
Let $L_{2D}=\{l\}$ denote the line segments in 2D, where $l=(s, e)$ is a tuple of start point $s \in \mathbb{S}^2$ and end point $e \in \mathbb{S}^2$.
Note that we express each point on a line from panorama images as a point on a unit sphere $\mathbb{S}^2$.
Similarly, let $L_{3D}=\{\tilde{l}\}$ denote the line segments in 3D, with $\tilde{l}=(\tilde{s}, \tilde{e})$ being a tuple containing start and end points $\tilde{s}, \tilde{e} \in \mathbb{R}^3$.
 
% The principal directions in 2D and 3D are estimated using vanishing point estimation and voting.
LDL estimates the vanishing point and votes for the principal directions in 2D and 3D.
For panorama images, vanishing points are extracted by finding the points of intersection for extended line segments.
The 2D principal directions $P_{2D}=\{p\}$ are defined as the top $k_{2D}$ vanishing points containing the most incident lines, where $p \in \mathbb{R}^3$ is a unit norm vector on a sphere denoting vanishing point location.
For point clouds, the 3D principal directions $P_{3D}=\{\tilde{p}\}$ are defined as the top $k_{3D}$ most common line directions from $L_{3D}$ obtained via voting.
Note that the 3D direction $\tilde{p} \in \mathbb{R}^3$ is also normalized.
\fi

\subsubsection{Candidate Rotation Estimation}
\label{sec:rotation}
LDL estimates the feasible candidate rotations up to uncertainty in the combinatorial ambiguities when matching the principal directions in 2D and 3D. % , as shown in Figure~\ref{fig:rotation}.
Specifically, we select triplets of directions from the principal directions $P_{2D}$ and $P_{3D}$, yielding a total of ${k_{2D}\choose 3} \times {k_{3D} \choose 3} \times {3!} \times {2^3}$ possible combinations, additionally considering the sign and permutation ambiguity.
For each pair of triplets, we apply the Kabsch algorithm~\cite{kabsch} to find the optimal rotation that aligns the 2D directions to 3D directions.
Discarding infeasible rotations that have large mean squared error, we obtain $N_r$ rotations.
The possible rotations are further filtered using line distance function presented in the next section.
% \input{figures/fig_rotation}

\input{figures/fig_ldf}
\subsubsection{Line Distance Functions for Pose Selection}
\label{sec:distance}
We propose line distance functions to efficiently evaluate a large pool of poses and select promising candidate poses.
The initial pool of poses are the combination of possible translations with the rotations found from the previous section. 
To this end, $N_t$ translations are chosen within grid partitions of the 3D point cloud, where details are explained in the supplementary material.
The resulting $N_t \times N_r$ poses are ranked using line distance functions.

\paragraph{Distance Function Definition} 
Distance functions are designed to compare the holistic spatial context captured from the large field of view in panorama images.
A line distance function is a dense field of distance values from a spherical projection of detected lines at each candidate pose in 3D and the 2D query image.
They are defined for every point including void regions without any lines and can quickly rank poses.
Compared to Chamfer distance or learned line embeddings used in prior work~\cite{line_chamfer,line_transformer}, 
LDL does not attempt pairwise matching between lines, which is often costly and can possibly incur failure modes.
For example, it is ambiguous to correctly match between densely packed lines as shown in Figure~\ref{fig:motivation}(a).

% Simplified notation for spherical distance
Let $L_{2D}=\{l\}$ denote the line segments in 2D, where $l=(s, e)$ is a tuple of start point $s \in \mathbb{S}^2$ and end point $e \in \mathbb{S}^2$.
Note that we express each point on a line from panorama images as a point on a unit sphere $\mathbb{S}^2$.
For a point $x \in \mathbb{S}^2$, the 2D line distance function is given as
\begin{equation}
	f_{2D}(x ; L_{2D}) = \min_{l \in L_{2D}} D(x, l).
\end{equation}
Here $D(x, l)$ is the spherical distance from $x$ to line segment $l=(s, e)$, namely
\begin{equation}
	D(x, l) = 
\left\{
	\begin{array}{lr}
		\sin^{-1} |\langle x, \dfrac{s \times e}{\|s \times e\|}\rangle|  &  \!\!\!\!\! \mbox{if $x \in \mathcal{Q}(s,e)$}\\
		\min (\cos^{-1} \langle x, e\rangle, \cos^{-1} \langle x, s\rangle) &  \!\!\!\!\! \mbox{otherwise,}
	\end{array}
\right.
\label{eq:line_dist}
\end{equation}
where $\mathcal{Q}(s,e)$ is the spherical quadrilateral formed from $\{s, e, \pm (s\times e) / \|s\times e\|\}$.

Similarly, let $L_{3D}=\{\tilde{l}\}$ denote the line segments in 3D, with $\tilde{l}=(\tilde{s}, \tilde{e})$ being a tuple containing start and end points $\tilde{s}, \tilde{e} \in \mathbb{R}^3$.
The 3D line distance function is defined for each candidate rotation $R \in SO(3)$ and translation $t \in \mathbb{R}^3$.
Using the spherical projection function $\Pi(\cdot): \mathbb{R}^{3}\rightarrow \mathbb{S}^{2}$ that maps a point in 3D to a point on the unit sphere, the 3D line segment $\tilde{l} = (\tilde{s}, \tilde{e})$ is projected to 2D under the candidate transformation as $l = (\Pi(R\tilde{s} + t), \Pi(R\tilde{e} + t))$.
For simplicity, let $\Pi_L (\tilde{l}; R, t)$ denote the projection of a line segment in 3D to the spherical surface.
Then the 3D line distance function is defined as follows,
\begin{equation}
	f_{3D}(x; L_{3D}, R, t) = \min_{\tilde{l} \in L_{3D}} D(x, \Pi_L(\tilde{l}; R, t)).
\end{equation}
As shown in Figure~\ref{fig:ldf}, one can expect poses closer to the ground truth to have similar 2D and 3D line distance functions.
Therefore, we evaluate $N_t \times N_r$ poses according to the similarity of line distance functions.

We apply a robust loss function that measures inlier counts to quantify the affinity of the line distance functions.
For each candidate pose $\{R, t\}$ we count the number of points whose distance function differs below a threshold $\tau$,
\begin{equation}
L(R, t) = \! - \!\! \sum_{q \in Q} \mathbbm{1}\{|f_{2D}(q; L_{2D}) - f_{3D}(q; L_{3D}, R, t)| < \tau\},
\label{eq:loss}
\end{equation}
where $\mathbbm{1}\{\cdot\}$ is the indicator function and $Q \subset \mathbb{S}^2$ is a set of query points uniformly sampled from a sphere.
The loss function from Equation~\ref{eq:loss} only considers inlier counts, and thus is robust to outliers from scene changes or line misdetections.
We validate the efficacy of the robust loss function in Section~\ref{sec:abl}.


\input{figures/fig_decomp}
\paragraph{Distance Function Decomposition}
To further enhance the pose search using line distance functions, we propose to decompose the distance functions into the three principal directions.
While line distance functions provide useful evidence for line-based localization, they lack a sense of direction as shown in Figure~\ref{fig:motivation}(b), where the distance functions alone cannot effectively distinguish rotated views from a fixed translation.

We split line segments along the principal directions used for rotation estimation and define separate line distance functions for each group of lines, as shown in Figure~\ref{fig:decomp}.
Recall that each candidate rotation $R$ is obtained from a pair of triplets in 2D and 3D principal directions, denoted as $\hat{P}_{2D}^R=\{p_1, p_2, p_3\}$ and $\hat{P}_{3D}^R=\{\tilde{p}_1, \tilde{p}_2, \tilde{p}_3\}$.
We associate line segments that are parallel to directions in $\hat{P}_{2D}^R, \hat{P}_{3D}^R$, leading to three groups of line segments $L_{2D}^R=\{L_{2D}^1, L_{2D}^2, L_{2D}^3\}$ and  $L_{3D}^R=\{L_{3D}^1, L_{3D}^2, L_{3D}^3\}$ in 2D and 3D, respectively.
We separately define line distance functions for the three groups using Equation~\ref{eq:line_dist}, namely $f_{2D}(x; L_{2D}^i)$ and $f_{3D}(x; L_{3D}^i, R, t)$ for $i = 1, 2, 3$.
Then the robust loss function in Equation~\ref{eq:loss} can be modified to accommodate the decomposed distance functions,
\begin{equation}
L(R, \! t) \! = \! - \!\!\sum_{i=1}^3\!\sum_{q \in Q} \!\mathbbm{1}\{|f_{2D}(q; \! L_{2D}^i) - f_{3D}(q;\! L_{3D}^i,\! R,\! t)| \!< \!\tau\}.
\label{eq:decomp}
\end{equation}
We validate the importance of distance function decomposition in Section~\ref{sec:abl}.

\subsection{Candidate Pose Refinement}
\label{sec:refinement}
As the final step, we select the top $K$ poses from the pool of $N_t \times N_r$ poses with the loss function values from Equation~\ref{eq:decomp}, and refine them.
Here we utilize the cached local features from Section~\ref{sec:input prep} and perform feature matching~\cite{sarlin2020superglue} followed by PnP-RANSAC~\cite{pnp_1,ransac}.
Specifically, for each selected pose we first retrieve the set of visible 3D keypoints at that pose and perform local feature matching against the 2D keypoints in the query image.
Here we use SuperGlue~\cite{sarlin2020superglue} for feature matching and select the candidate pose with the most matches.
We finally apply PnP-RANSAC~\cite{ransac, epnp} on the matched 2D and 3D keypoint coordinates to obtain a refined pose estimate.

\subsection{Privacy-Preserving Line-Based Localization}
\label{sec:privacy}
In this section, we describe how LDL can be used for privacy-preserving localization.
As many edge devices have limited compute, location-based services on edge devices employ a client-server localization setup where the visual data of the edge device is shared with the service provider~\cite{privacy_analysis, pittaluga_revealing}.
We consider three parties (mapper client, query client, and service provider) for our client-server localization setup, as shown in Figure X.

\paragraph{Mapper and Query Client} The mapper and query client extracts and shares the 2D, 3D line data with the service provider.
To elaborate, mapper client is the user that makes the 3D measurements of the scene using conventional 3D sensors~\cite{matterport_scan, faro_scan} (Figure X-(a)).
Using the raw 3D scans, the mapper client processes the data as explained in Section~\ref{sec:input prep}, namely 3D line detection and local feature extraction near lines, and shares the results with the service provider.
Query client is the edge device user that aims to localize oneself in the same scene as the mapper client (Figure X-(b)).
The query client client only performs 2D line detection and local feature extraction near lines and sends the results to the service provider.

\paragraph{Service Provider and Privacy Protection} Using the shared 2D and 3D line data, the service provider performs the main localization pipeline (Section~\ref{sec:rotation}-~\ref{sec:refinement}) and returns the 6DoF pose to the query client.
Privacy breaches occur if the service provider can have access to the sensitive visual information viewed by the clients.

In conventional visual localization~\cite{sarlin2019coarse,sarlin2020superglue}, breaches can happen amidst candidate pose selection and pose refinement.
During candidate pose selection, sharing the entire image view may be necessary as many localization methods employ global feature extractors~\cite{netvlad,robust_retrieval} that take the whole image as input.
For pose refinement, the service provider may try to reconstruct the client's view using the shared local features~\cite{pittaluga_revealing,ninjadesc}.
To elaborate, given a sparse feature map $D \in \mathbb{R}^{H \times W \times C}$ containing local descriptors at keypoint locations, service providers can use feature inversion methods~\cite{ninjadesc, pittaluga_revealing, privacy_analysis} that learn a neural network $F_\Theta(\cdot)$ to recover the original image $I$, namely $F_\Theta(D) = I$.

Due to the line-based paradigm, LDL offers privacy protection in all stages of localization.
First, as LDL only uses line segments for candidate pose selection, it does not necessitate the clients to share their entire view with the service provider.
Second, as local features near line segments are shared with the service provider, feature inversion methods~\cite{ninjadesc, pittaluga_revealing} cannot fully recover the original visual content.
LDL only considers long line segments conforming to the principal directions, and thus local features from sensitive entities such as people and tabletop clutter are removed prior to sharing.
We further validate the privacy protection of LDL in Section 4-X.


==> tables/rebuttal_iccv_tab.tex <==
\begin{table}[t]
\centering
    \begin{subtable}{0.44\linewidth}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccc}
        \toprule
        Method & $t$-error (m) & $R$-error ($^\circ$) & Acc.\\
        \midrule
        SfM & \textbf{0.03} & 0.80 & 0.85\\
        3D Scan & \textbf{0.03} & \textbf{0.71} & \textbf{0.98} \\
        \bottomrule
    \end{tabular}
    }
    \caption{Evaluation on Noisier Maps}
    \label{table:reb_iccv_noise}
    \end{subtable}
    \smallskip
    \begin{subtable}{0.53\linewidth}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccc}
        \toprule
        Method & $t$-error (m) & $R$-error ($^\circ$) & Acc.\\
        \midrule
        LDL & \textbf{0.02} & \textbf{0.54} & \textbf{0.90}\\
        Structure-Based & 0.03 & 0.58 & 0.89 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Evaluation on Large Scale Scenes }
    \label{table:reb_iccv_scale}
    \end{subtable}

    \caption{Additional quantitative evaluation results of LDL.}
    \label{table:reb_iccv}

\end{table}


==> tables/rebuttal_line_filter.tex <==
\begin{table}[t]
\centering
    \centering
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{ll|cccc}
        \toprule
        Attack & Method & 20-PSNR & 1-SSIM & MAE  \\
        \midrule
        \multirow{2}{*}{2D Inversion} & No Filtering & 0.7339 & 0.5302 & 0.1577 \\
        & Filtering & \textbf{2.0727} & \textbf{0.5917} & \textbf{0.1902} \\
        \bottomrule
    \end{tabular}
    }
\vspace{-0.5em}
\caption{Privacy-preservation evaluation against feature inversion networks trained on features near lines. }
\label{table:rebuttal_line_attack}
\vspace{-1em}
\end{table}

==> tables/rebuttal_multi_room.tex <==
\if 0
\begin{table}[t]
\centering
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{l|ccc}
    \toprule
    Method &  Acc. & Loc. Runtime & Feat. Runtime \\
    \midrule
    SB & 0.99 & 0.XX & 0.XX\\
    SB (Perspective) & 0.99 & 0.XX & 0.XX\\
    Ours & 0.99 & 0.XX & 0.XX\\
    \bottomrule
\end{tabular}
}
\vspace{-0.5em}
\caption{Performance comparison on multiple-room settings.}
\label{table:rebuttal_multi_room}
\vspace{-1em}
\end{table}
\fi

\begin{table}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{ll|ccc}
    \toprule
    Setup & Method &  Acc. & Loc. Runtime & Feat. Runtime \\
    \midrule
    \multirow{3}{*}{Original} & SB (View Cropping) & \textbf{0.92} & 5.673 & 175.932\\
    & SB (Larger Trans.) & \textbf{0.92} & 0.773 & 1854.242\\
    & Ours & 0.84 & \textbf{0.089} & \textbf{8.143}\\
    \midrule
    \multirow{2}{*}{\begin{tabular}{@{}l@{}}Multiple \\ Rooms\end{tabular}} & SB & 0.71 & 0.762 & 900.48\\
    & Ours & \textbf{0.72} & \textbf{0.604} & \textbf{36.16}\\
    \bottomrule
\end{tabular}
}
\vspace{-0.5em}
\caption{Comparison with structure-based methods (SB). Accuracy is computed with $0.1\text{m}$, $5^\circ$ threshold. We also report runtimes for localization and feature preparation prior to localization.}
\label{table:rebuttal_structure_based}
\vspace{-1em}
\end{table}

==> tables/rebuttal_sb_acc.tex <==
\begin{table}[t]
\centering
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{l|ccc}
    \toprule
    Method &  Acc. & Loc. Runtime & Feat. Runtime \\
    \midrule
    View Cropping & 0.99 & 0.XX & 0.XX\\
    Larger Trans. & 0.99 & 0.XX & 0.XX\\
    Ours & 0.99 & 0.XX & 0.XX\\
    \bottomrule
\end{tabular}
}
\vspace{-0.5em}
\caption{Comparison with structure-based methods (SB). Accuracy is computed with $0.1\text{m}$, $5^\circ$ threshold. We also report runtimes for localization and feature preparation prior to localization.}
\label{table:rebuttal_sb}
\vspace{-1em}
\end{table}


==> tables/tab_loc_eval.tex <==
\begin{table*}[t]
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{l|cccccc|cccccc|cccccc}
        \toprule
        {} & \multicolumn{6}{c|}{$t$-error (m)} & \multicolumn{6}{c|}{$R$-error ($^\circ$)} & \multicolumn{6}{c}{Accuracy}\\
        Dataset & PC & SB & CD & LT & CPO & LDL & PC & SB & CD & LT & CPO & LDL & PC & SB & CD & LT & CPO & LDL \\
        \midrule
        Stanford 2D-3D-S & 0.03 & 0.04 & 0.73 & 0.03 & \textbf{0.01} & 0.02 & 0.63 & 0.76 & 2.30 & 0.77 & \textbf{0.24} & 0.53 & 0.54 & 0.61 & 0.39 & 0.61 & \textbf{0.83} & \textbf{0.83} \\
        \midrule
        OmniScenes (No Change) & 0.01 & 0.03 & 1.96 & 0.03 & \textbf{0.01} & 0.03 & 0.24 & 0.58 & 89.10 & 0.58 & \textbf{0.12} & 0.54 & 0.76 & 0.86 & 0.30 & 0.88 & 0.84 & \textbf{0.93} \\
        OmniScenes (Change) & 0.99 & 0.04 & 1.67 & 0.04 & \textbf{0.02} & 0.03 & 18.15 & 0.75 & 88.91 & 0.72 & 1.13 & \textbf{0.67} & 0.44 & 0.75 & 0.30 & 0.79 & 0.59 & \textbf{0.86} \\

        \bottomrule
    \end{tabular}
    }
    \vspace{-0.5em}
    \caption{Localization performance evaluation in Stanford 2D-3D-S~\cite{stanford2d3d} and OmniScenes~\cite{piccolo}. Our method is compared against PICCOLO (PC)~\cite{piccolo}, structure-based approach (SB), Chamfer distance-based approach (CD), Line Transformer (LT)~\cite{line_transformer}, and CPO~\cite{cpo}.}
    \label{table:stanford}
\vspace{-1em}
\end{table*}


==> tables/tab_privacy.tex <==
\begin{table}[t]
\begin{subtable}{\linewidth}
    \centering
    \resizebox{0.55\linewidth}{!}{
    \begin{tabular}{l|cccc}
        \toprule
        Method & $t$-error (m) & $R$-error ($^\circ$) & Acc.\\
        \midrule
        No Filtering & \textbf{0.02} & \textbf{0.53} & \textbf{0.83} \\
        Filtering & 0.03 & 0.64 & 0.77 \\
        \bottomrule
    \end{tabular}
    }
\caption{Localization Performance Evaluation}
\end{subtable}

\smallskip

\begin{subtable}{\linewidth}
    \centering
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{ll|cccc}
        \toprule
        Attack & Method & 20-PSNR & 1-SSIM & MAE  \\
        \midrule
        \multirow{2}{*}{2D Inversion} & No Filtering & 1.1717 & 0.5505 & 0.1598 \\
        & Filtering & \textbf{1.7577} & \textbf{0.6027} & \textbf{0.1773} \\
        \midrule
        \multirow{2}{*}{3D Inversion} & No Filtering & 2.4432 & 0.6774 & 0.1957 \\
        & Filtering & \textbf{3.3606} & \textbf{0.7406} & \textbf{0.2240} \\
        \bottomrule
    \end{tabular}
    }
\caption{Reconstruction Quality of 2D, 3D Inversion Attacks}
\end{subtable}
\vspace{-1em}
\caption{Privacy-preservation evaluation of line-based feature filtering on a fixed filtering threshold $\lambda_{2D}{=}0.05\text{ rad}, \lambda_{3D}{=}0.1\text{ m}$. }
\label{table:preservation}
\vspace{-1em}
\end{table}
